Design and Analysis of Efficient Maximum/Minimum Circuits for Stochastic Computing

In stochastic computing (SC), a real-valued number is represented by a stochastic bit stream, encoding its value in the probability of obtaining a one. This leads to a significantly lower hardware effort for various functions and provides a higher tolerance to errors (e.g., bit flips) compared to binary radix representation. The implementation of a stochastic max/min function is important for many areas where SC has been successfully applied, such as image processing or machine learning (e.g., max pooling in neural networks). In this work, we propose a novel shift-register-based architecture for a stochastic max/min function. We show that the proposed circuit has a significantly higher accuracy than state-of-the-art architectures at comparable hardware cost. Moreover, we analytically proof the correctness of the proposed circuit and provide a new error analysis, based on the individual bits of the stochastic streams. Interestingly, the analysis reveals that for a certain practical bit stream length a finite optimal shift register length exists and it allows to determine the optimal length.

==> LinearFSM.tex <==
% ===================================================================
% File: LinearFSM.tex
% Desc.: Main properties of linear FSMs
% Created: 24.01.2018, wh
% Changed: 
% ===================================================================

Fig. \ref{} shows a linear finite state machine, with $N$ states $S_0,\dots S_{N-1}$ arranged in 
a linear form. The state transition process of the FSM can be modeled as a time-homogeneous irreducible and aperiodic Markov chain which 
has a single steady state \cite{}. In the steady state, the probability of transitioning from state  $S_{i-1}$ to $S_i$ must be equal to the probability of 
transitioning  from $S_i$ to $S_{i-1}$, which can be formulated as follows
\begin{align}
  P_{i-1} P_X = P_i P_Y, \quad i=0,\ldots, N-1,
\end{align}

where $P_i$ denotes the probability of the $i$th state. Through recursive substitution the state probability 
can be expressed as
\begin{align}
  P_i = \frac{\left(\frac{P_X}{P_Y}\right)^i}{\sum\limits_{j=0}^{N-1} \left(\frac{P_X}{P_Y}\right)^j},
  \label{eq:steady_state_prob}
\end{align}

where the expression in the denominator corresponds to a normalization, since in the steady state the individual probability must to unity. The output of the state machine is only determined by the current state and can be expressed as follows
\begin{align}
  P_Z = \sum\limits_{i=0}^{N-1} s_i P_i,
  \label{eq:fsm_output_general}
\end{align}

with $s_i \in \{0,1\}$. Through different settings of $s_i$ the linear FSM allows the realization of many arithmetic functions, such as stochastic exponential function, stochastic tanh function or a stochastic gain function \cite{}. In the following, we briefly review the stochastic tanh function, since this is a main building block for the stochastic min/max functions\footnote{Please refer to \cite{Brown_01,Li_14} for more details.} presented in the next sections. For the tanh function the parameters $s_i$ in \eqref{eq:fsm_output_general} are set as follows \cite{Brown_01}
\begin{align}
  s_i = \begin{cases}
                s_i = 0, \quad 0 \leq i < N/2-1 \\
                s_i = 1, \quad N/2 \leq i \leq N-1.
         \end{cases}
\end{align}

Thus, the FSM output is given by 
\begin{align}
  P_Z = \sum\limits_{i=N/2}^{N-1} s_i P_i,
  \label{eq:fsm_output_tanh}
\end{align}


Substituting $P_i$ given in \eqref{eq:steady_state_prob}, with  $P_Y = 1-P_X$, into \eqref{eq:fsm_output_tanh} results in~\cite{Li_14}
\begin{align}
  P_Z %= \frac{\left(\frac{P_X}{P_Y}\right)^{N/2}}{1 + \left(\frac{P_X}{P_Y}\right)^{N/2}} 
      = \frac{\left(\frac{P_X}{1-P_X}\right)^{N/2}}{1 + \left(\frac{P_X}{1-P_X}\right)^{N/2}},
  \label{eq:fsm_output_tanh_1}
\end{align}

For a large number of states in the FSM, the output $P_Z$ behaves like a step function
\begin{align}
  \mathop{\text{lim}}_{N\rightarrow \infty} P_Z = 
                                           \begin{cases}
                                             P_Z = 0, & 0 \leq P_X < 0.5 \\
                                             P_Z = 0.5, & P_X=0.5\\
                                             P_Z = 1, & 0.5 < P_X \leq 1.
                                           \end{cases}
  \label{eq:fsm_output_tanh_limit}
\end{align}

For the bipolar format we substitute $P_X$ and $P_Z$ by $(x+1)/2$ and  $(z+1)/2$, respectively. Now, for the FSM output we have~\cite{Li_14}
\begin{align}
  z & = \frac{\left(\frac{x}{1-x}\right)^{N/2}}{1 + \left(\frac{x}{1-x}\right)^{N/2}} 
        \approx \frac{e^{\frac{N}{2}x} - e^{-\frac{N}{2}x} }{e^{\frac{N}{2}x} + e^{-\frac{N}{2}x}} = \text{tanh}\left(\frac{N}{2}x\right).
\end{align}

and in case of a large number states $N$ we obtain
\begin{align}
  \mathop{\text{lim}}_{N\rightarrow \infty} z = \begin{cases}
                                           z=-1, & -1 \leq x < 0 \\
                                           z=0, & x = 0\\
                                           z = 1, & 0 < x \leq 1.
         \end{cases}
\end{align}

%Fig. \ref{} shows the tanh function for different FSM lengths. \todo[inline]{Fig. with 3-4 curves; subfigure?}

For the unipolar format  we substitute $P_X$ and $P_Z$ by $x$ and  $z$, respectively. Now, for the FSM output we have
\begin{align}
  z & = \frac{\left(\frac{x}{1-x}\right)^{N/2}}{1 + \left(\frac{x}{1-x}\right)^{N/2}}
        \approx \frac{1 + \text{tanh}\left(N/2\left(x - 1/2\right)\right)}{2},
\end{align}

and for a large number of states $N$ we obtain
\begin{align}
  \mathop{\text{lim}}_{N\rightarrow \infty} z = \begin{cases}
                                           z=0, & 0 \leq x < 0.5 \\
                                           z=0.5, &  x = 0.5 \\
                                           z = 1, &  0.5 < x \leq 1.
         \end{cases}
\end{align}

%Fig. \ref{} shows this function for different FSM lengths.\todo[inline]{Fig. with 3-4 curves; subfigure?}


==> PerformanceAnalysis.tex <==
% ===================================================================
% File: PerformanceAnalysis.tex
% Desc.: Performance Analysis of the proposed stochastic inner product
% Created: 23.05.2018, wh
% Changed: 
% ===================================================================

% Figures on the computational complexity (which platform was used to evaluate 
% the number of required logic elements and registers). 
% Do we have some numbers for the possible clock frequency.
% Compare complexity without synchronization circuitry (assume that the clocks are synchronized)
% Figure on the fault tolerance

% ---------------------------
% Make two separate figures!!
\begin{figure*}[t!]
	\centering
	\includegraphics[scale=0.4]{complexity_comparison}
	\caption{Implementation complexity comparison of different inner product implementations. Errors are defined as $\sqrt{\text{mean}\vert\hat{x} - x\vert^2}$. Blue squares are hidden behind orange and green ones.}
	\label{fig:complexity_comparison}
\end{figure*}
% ---------------------------

In this section, we compare the proposed inner product implementation with the state-of-the-art stochastic implementation and a sequential fixed-point realization. The state-of-the-art stochastic implementation consists of signed magnitude multipliers and an adder-tree of counter-based non-scaled adders, that have been proposed in \cite{7560185, 7553519}.
The fixed-point implementation uses the s1.F format and processes its inputs sequentially. Hence, it just uses a single multiplier and an adder. Please note, that the deterministic inputs of stochastic bitstream generators must be constant, while the stochastic bitstreams are being generated and, in further consequence, being processed. To enable a fair comparison, this is also assumed for the fixed-point case. Hence, the fixed-point implementation's deterministic input values are assumed to be constant and do not have to be stored in input registers.\\

\fig{fig:complexity_comparison} presents the minimum number of logic elements/registers, that are required, to make an implementation achieve a certain accuracy. The stochastic implementations' bitstream length is fixed ($N = 10000$). Hence, their accuracy is only controlled by varying their carry shift register or carry counter lengths. For the fixed-point implementation, the accuracy is controlled by varying the bit width.\\

When investigating the logic element utilization, the state-of-the-art stochastic implementation is very inefficient in terms of hardware effort, especially for large input vector lengths and a high calculation accuracy. For an input vector length of $64$ and an error of $\sqrt{\text{mean}\vert\hat{x} - x\vert^2} \leq 0.02$, an amount of $2034$ logic elements is required. The novel stochastic implementation, on the other hand, achieves the same task with only $355$ logic elements. This is a saving of \SI{83}{\%}. When investigating the register utilization, for the given use cases, the state-of-the-art stochastic implementation is better. It does not require synchronization circuitry (e.g. input hold registers) or sequential processing storage (input shift registers). However, while the novel implementation's resource utilization is almost independent of the required calculation accuracy, the state-of-the-art implementation's register utilization is not. This makes the state-of-the-art implementation's register count exceed the novel implementation's register count, when the required calculation accuracy becomes sufficiently high. For an error of $\sqrt{\text{mean}\vert\hat{x} - x\vert^2} \leq 0.02$, the novel implementation's register count is only about 21 registers larger than the register count of the state-of-the-art implementation. This further improves, if the novel implementation's clocks are synchronized. In that case, its synchronization circuitry can be omitted.\\

The novel stochastic implementation is also very competitive, when its hardware effort is compared to the one of the fixed-point realization. For the discussed use case, the novel stochastic implementation saves $594$ logic elements, where the fixed-point implementation's multiplier logic has not even been counted. In case of register usage, the fixed-point implementation is clearly more efficient. This is, because it does not require any synchronization circuitry or adder-internal carry storage.\\

As stated before, the novel stochastic implementation's complexity is nearly constant over accuracy. This is a unique feature of the proposed implementation and enables us to control the system's accuracy by only varying the bitstream length.

Another feature is the novel implementation's relatively high robustness against bit flips. Due to the implementations' architectural differences and the high-level models' abstractions, a robustness quantification is challenging. However, robustness can be roughly estimated by randomly flipping an implementation's storage bits and by observing the calculation error, that results. \fig{fig:robustness_comparison} presents the results of this investigation. By using an input vector length of $16$ and configuring the implementations to start from nearly equal calculation errors of $\sqrt{\mathrm{mean}\vert\hat{x}-x\vert^2} \approx 0.02$, it presents the respective errors over the probability, that a certain storage bit flips. For the stochastic implementations, the bitstream length has again been set to 10000.\\ 

% ---------------------------
\begin{figure}[t!]
	\centering
	\includegraphics[scale=0.6]{robustness_comparison}
	\caption{Robustness comparison of the novel stochastic and state-of-the-art stochastic/fixed-point inner product implementations.}
	\label{fig:robustness_comparison}
\end{figure}
% ---------------------------

As indicated, the novel stochastic implementation's calculation errors are much smaller than the other ones', implying, that it is more robust against bit flips. This is a plausible result, since it does not use the bit-flip-vulnerable conventional binary representation of the fixed-point and state-of-the-art stochastic system.

